Structure Theorem and Isomorphism Test for Graphs with Excluded Topological Subgraphs

We generalize the structure theorem of Robertson and Seymour for graphs excluding a fixed graph $H$ as a minor to graphs excluding $H$ as a topological subgraph. We prove that for a fixed $H$, every graph excluding $H$ as a topological subgraph has a tree decomposition where each part is either "almost embeddable" to a fixed surface or has bounded degree with the exception of a bounded number of vertices. Furthermore, we prove that such a decomposition is computable by an algorithm that is fixed-parameter tractable with parameter $|H|$. We present two algorithmic applications of our structure theorem. To illustrate the mechanics of a "typical" application of the structure theorem, we show that on graphs excluding $H$ as a topological subgraph, Partial Dominating Set (find $k$ vertices whose closed neighborhood has maximum size) can be solved in time $f(H,k)\cdot n^{O(1)}$ time. More significantly, we show that on graphs excluding $H$ as a topological subgraph, Graph Isomorphism can be solved in time $n^{f(H)}$. This result unifies and generalizes two previously known important polynomial-time solvable cases of Graph Isomorphism: bounded-degree graphs and $H$-minor free graphs. The proof of this result needs a generalization of our structure theorem to the context of invariant treelike decomposition.

==> structure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Structure Theorem}

\begin{theo}\label{theo:structure}
  For every $k\in\NN$, there exists constants $a(k)$, $b(k)$, $c(k)$,
  $d(k)$, $e(k)$, such that the following holds. Let $H$ be a graph on
  $k$ vertices. Then for every graph $G\in\CX_T(H)$ there is a tree
  decomposition $(T,\bag)$ of adhesion at most $a(k)$ such that for
  all $t\in V(T)$ one of the following three conditions is satisfied:
  \begin{eroman}
  \item $|\bag(t)|\le b(k)$.
  \item $\tau(t)$ has at most $k$ vertices of degree larger than $d(k)$.
  \item $K_{e(k)}\not\preceq\tau(t)$.
  \end{eroman}
  Furthermore, there is an algorithm that, given graphs $G,H$ of sizes
  $n,k$, respectively, in time $f(k)\cdot n^{O(1)}$ for some
  computable function $f$, computes either such a decomposition
  $(T,\beta)$ or a subdivision of $H$ in $G$.
\end{theo}

% The theorem, at least without the algorithmic part, follows from our previous
% lemmas and Theorem (11.1) of \cite{gm10}. However, since the terminology used
% in \cite{gm10} is quite different from ours and since we need to prove the algorithmic claim anyway, we
% describe the construction without explicit reference to \cite{gm10}.

\begin{proof}[Proof of Theorem~\ref{theo:structure}]
  Let $k:=|H|$ and let $a(k)$, $b(k)$, $c(k)$, $d(k)$, $e(k)$ as in
  Lemma~\ref{lem:mainstar}.  Let $G$ be a graph. We shall describe the
  construction of a tree decomposition $(T,\bag)$ of $G$ satisfying
  all conditions asserted in the lemma. The construction may fail, but
  in that case it yields a toplogical minor image of $H$ in $G$.
 % We
 %  will show that the construction leads to an algorithm with the
 %  desired running time afterwards.

  We will built the tree $T$ inductively starting from the root. For every
  node $t$ we will define the set $N^T(t)$ of its children and sets
  $\sep(t),\comp(t)$ such that $|\sep(t)|\le a(k)$ and $N^G(\comp(t))\subseteq\sep(t)$. As usual, we define $\cone(t)$,
  $\bag(t)$, and $\tau(t)$ as in \eqref{eq:cone}, \eqref{eq:bag}, and
  \eqref{eq:torso}. In each step, we will prove that
  $\tau(t)$ satisfies one of (i), (ii), or (iii).


  We start with a root $r$ of $T$ and let $\sep(r):=\emptyset$ and
  $\comp(r):=V(G)$. For the inductive step, let $t$ be a node for
  which $\sep(t)$ and $\comp(t)$ are defined, but $N^D(t)$ is not yet
  defined. We let $G_t:=G[\cone(t)]$.  
% If $|\cone(t)|\le b(k)$, we let
%   $N^D(t):=\emptyset$ and stop, as $\tau(t)$ has maximum degree $b(k)\le d'$.
%   Otherwise, 
  Let us run the algorithm of Lemma~\ref{lem:mainstar} on $G_t$ (as
  $G$), $\sep(t)$ (as $S$), and $k$. If it returns a subdivision of
  $K_k$ in $G_t$, then we can clearly return as subdivision of $H$ in
  $G$ and we are done. Otherwise, it returns a start decomposition
  $\Sigma_t:=(T_t,\sep_t,\comp_t)$ of $G\cup K_{\sep(t)}$ having adhesion at most $a(k)$; let $r_t$
  be the centre of $T_t$. We let $N^T(t):=V(T_t)\setminus\{r_t\}$ be
  the set of tips of $T_t$, where without loss of generality we assume
  that this set is disjoint from the tree $T$ constructed so far. For
  every $u\in N^T(t)$ we let $\sep(u):=\sep_t(u)$ and
  $\comp(u):=\comp_t(u)$.  Observe that we have
  $\bag(t)=\cone(t)\setminus\bigcup_{u\in
    N^T(t)}\comp(u)=\bag_t(r_t)$.  Furthermore, since $\Sigma_t$ is a
  decomposition of $G\cup K_{\sep(t)}$ and $\sep(t)$ induces a clique
  in $G\cup K_{\sep(t)}$, we have that $\torso(t)=\torso_t(r_t)$.
  Thus one of the three cases of Lemma~\ref{lem:mainstar} holds for
  the bag $\bag(t)$ as well.

  To see that $(T,\bag)$ is a tree decomposition, it is easiest to
  verify it satisfies \ref{li:t2}--\ref{li:t4}: it follows from the
  fact that the star decomposition $\Sigma_t$ used in each step of the
  construction does satisfy these conditions. Condition \ref{li:t1} is
  obvious and \ref{li:t5} follows because we start the construction
  with a node $t$ having $\comp(t)=V(G)$ and $\sep(t)=\emptyset$.
  Note that the bound $a(k)$ on the adhesion of $\Sigma_t$ implies the
  same bound on the adheasion of $(T,\bag)$.

  To see that the construction terminates, note that for all $t\in
  V(T)$, Lemma~\ref{lem:mainstar} states that $\comp_t(u)\subset
  \comp_t(r_t)$ for every tip $u$ of $T_t$. Therefore, for every $u\in
  N^T(t)$, it holds that $\comp(u)\subset \comp(t)$.  Therefore, the
  height of the tree is at most $|V(G)|$.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "invdec"
%%% End: 

